The addition of temporal neighborhood makes the logic of prefixes and sub-intervals EXPSPACE-complete

A classic result by Stockmeyer gives a non-elementary lower bound to the emptiness problem for star-free generalized regular expressions. This result is intimately connected to the satisfiability problem for interval temporal logic, notably for formulas that make use of the so-called chop operator. Such an operator can indeed be interpreted as the inverse of the concatenation operation on regular languages, and this correspondence enables reductions between non-emptiness of star-free generalized regular expressions and satisfiability of formulas of the interval temporal logic of chop under the homogeneity assumption. In this paper, we study the complexity of the satisfiability problem for suitable weakenings of the chop interval temporal logic, that can be equivalently viewed as fragments of Halpern and Shoham interval logic. We first consider the logic $\mathsf{BD}_{hom}$ featuring modalities $B$, for \emph{begins}, corresponding to the prefix relation on pairs of intervals, and $D$, for \emph{during}, corresponding to the infix relation. The homogeneous models of $\mathsf{BD}_{hom}$ naturally correspond to languages defined by restricted forms of regular expressions, that use union, complementation, and the inverses of the prefix and infix relations. Such a fragment has been recently shown to be PSPACE-complete . In this paper, we study the extension $\mathsf{BD}_{hom}$ with the temporal neighborhood modality $A$ (corresponding to the Allen relation \emph{Meets}), and prove that it increases both its expressiveness and complexity. In particular, we show that the resulting logic $\mathsf{BDA}_{hom}$ is EXPSPACE-complete.

==> aregexp.tex <==
%!Tex root = ./main.tex

\section{Adding modality \texorpdfstring{$\mathtt{A}$}\ \ to \texorpdfstring{$\mathsf{BD}_{hom}$}{}: the logic \texorpdfstring{$\mathsf{BDA}_{hom}$}{}}
\label{sec:aregexp}

In this section, we introduce the logic $\mathsf{BDA}_{hom}$, that extends $\mathsf{BD}_{hom}$ with modality $\hsEA$. The semantics of modality $\hsEA$ has been already given in Section~\ref{sec:itlintro} in terms of modality $\cdtT$ of $\mathsf{CDT}$ as $\hsEA\psi = \psi \cdtT \top$. Formally, syntax and semantics of $\mathsf{BDA}_{hom}$ are obtained from those of $\mathsf{BD}_{hom}$ by simply adding the syntactic rule and the semantic clause for modality $\hsEA$, respectively.

$\mathsf{BDA}_{hom}$ formulas are built up from a countable set $\Prop$ of proposition letters according to the grammar:
$
\varphi ::= p\ |\ \neg \psi\ |\  \psi \vee \psi \ |\ 
\hsEB \psi \ |\ \hsED \psi \ |\ \hsEA \psi,
$
where $p \in \Prop$ and $\hsEB$, $\hsED$, and $\hsEA$ are the modalities for Allen's relations \emph{Begins}, \emph{During}, and \emph{Meets}, respectively.

The semantics of a $\mathsf{BDA}_{hom}$ formula
is specified by the semantic clauses for $\mathsf{BD}_{hom}$ 
plus the following one:
\\
\begin{compactitem}
\item $\bfM, [x,y] \models \hsEA \psi$ iff 
there is $y'$, with $y'\geq y$, such that
$\bfM, [y,y']\models \psi$.
\end{compactitem}
\vspace{0.45cm}

In the rest of section, in analogy to what we did for modalities $\hsEB$ and $\hsED$ in Section~\ref{sec:logic}, we investigate the counterpart of 
modality $\hsEA$ in terms of a suitable extension of generalized $*$-free regular expressions. Basically, we enrich the semantics of generalized $*$-free regular expressions with what we call a ``right context''. We will prove that the resulting semantics subsumes the original one, that is, the notion of generalized $*$-free regular expression given in Section~\ref{sec:logic} is just a specialization of it. In particular, 
the encoding of both $\Pre(e)$ and $\Sub(e)$ directly transfers to this
new semantics without any modification. We will conclude the section by 
providing an example that shows how the operator corresponding  to modality $\hsEA$ has an explicit counterpart in the generalized $*$-free regular expressions used 
for real-world programming languages.  

As a preliminary remark, we would like to observe that one may be tempted to interpret modality $\hsEA$ as a logical counterpart of the concatenation operator. This is wrong. Informally speaking, modality $\hsEA$ characterizes words with a specific ``right context''.
%the words of languages which appear to have a specific ``right context''. 
Such an idea can be formalized as follows.

In order to identify the right generalized $*$-free regular 
expression for modality $\hsEA$, we provide an alternative, yet 
equivalent, semantics for these expressions. In such a semantics, the 
language $\Rlang(e)$ of a generalized $*$-free regular expression $e$ is interpreted over pairs 
of finite words, that is, $\Rlang(e) \subseteq \Sigma^+ \times \Sigma^*$.
A pair $(w,w') \in \Rlang(e)$ represents the word $w$ belonging to the language $\Lang(e)$, according to the semantics given in  Section~\ref{sec:logic}, together with its ``right context'' word $w'$, which is the word that must appear immediately after $w$. 

\smallskip

Formally, generalized $*$-free regular expressions of Section~\ref{sec:logic} are extended as follows:
\[ e ::= \emptyset \ |\ a\ |\ \neg e\ |\ e + e \ |\ \ \Pre(e)\ 
|\ \Sub(e)\ |\  \Rcon(e),
   \mbox{ for any $a \in \Sigma$}
\]
Their semantics is defined as follows: 

\smallskip

\begin{compactenum}[(i)]
\item $\Rlang(\emptyset) = \emptyset$;
\item $\Rlang(a) = \{ (a, w): w \in \Sigma^* \}$;
\item $\Rlang(\neg e) =  \Sigma^+ \times \Sigma^* \setminus  \Rlang(e)$;
\item $\Rlang(e + e') =  \Lang(e) \cup \Lang(e')$;
\item $\Rlang(\Pre(e)) =  \{(wv, u): v \in \Sigma^+, (w, vu) \in \Rlang(e)  \}$;
\item $\Rlang(\Sub(e)) =  \{(uwv, z): u, v \in \Sigma^+, (w, vz) \in \Rlang(e) \}$;
\item $\Rlang(\Rcon(e)) =  \{(w, u): u \in  \Rlang(e) \}$.
\end{compactenum} 

Let us denote the empty word by $\epsilon$. With a little abuse of
notation, we say that, for every $w \in \Sigma^+$, $w \in \Lang(e)$  if and only if $(w,\epsilon) \in \Rlang(e)$. Then, it is easy to prove that, for any expression $e ::= \emptyset \ |\ a\ |\ \neg e\ |\ e + e \ |\ \ \Pre(e)\ |\ \Sub(e)$, $w \in \Lang(e)$ if and only if $(w, \epsilon) \in \Rlang(e)$.
In such a way, the original (restricted) semantics turns out to be a specialization of the extended one. 

It can be easily shown that the extended semantics preserves the 
%interval temporal logic 
mapping from a restricted expression $e$ to an equivalent $\mathsf{BD}_{hom}$ formula $\varphi_e$ outlined in 
Section~\ref{sec:logic}. In order to capture the language $\Rlang(\Rcon(e))$ in $\mathsf{BDA}_{hom}$, we extend the mapping with the rule:
$$
\varphi_{\Rcon(e)} = \hsEA(\hsEB \top \wedge 
\hsAB\hsAB \bot \wedge \hsEA \psi_e ).
$$
Let us assume that $\varphi_{\Rcon(e)}$ holds over an interval $[x,y]$. Then, it predicates over ``the right context'' of $[x,y]$ by stating that there exists an interval $[y,y+1]$ (the constraint on the length of such an interval is imposed by the first two conjuncts $\hsEB \top \wedge \hsAB\hsAB \bot$) which has an adjacent-to-the-right interval $[y+1, y']$ where $\psi_e$ holds
(third conjunct $\hsEA \psi_e$).

\smallskip

% example 
% please refer to https://regex101.com for a more comprehensive list 
% (\w+)(?= (?:\w+, ){2,}and \w+)
% This paper deals with HS operators meets, begins, ends, and during under homogeneity assumption.
% python relation with lookahead

In order to show the significance of the proposed extension of generalized $*$-free regular expression, we explore an interesting correspondence between the operator $\Rcon$ (and thus, indirectly, modality $\hsEA$) and an operator of the regular expressions tipically used in popular programming languages like, for instance, Python \cite{van1995python}. 
It is easy to see that the $\Rcon$ operator corresponds to the \emph{lookahed operation}. Such an operation is usually 
implemented as \emph{positive lookahead}, whose syntax is 
$\mathtt{(?= \mathbf{e} )}$, and \emph{negative lookahed},
whose syntax is $\mathtt{(?\ !\ \mathbf{e} )}$, where $e$ is a regular 
expression. In many real-world applications, regular expressions are used to execute \emph{pattern matching} inside a long text as an effective alternative to the task of checking whether such a long text belongs to a certain language. This is 
the case especially in the domain of natural language processing from 
which the following toy example is borrowed. Let us suppose that we 
want to capture a pattern that consists of an English word followed 
by a list of words in English separated by commas and whose last word is 
prefixed by the word \emph{``and''}. An example of a sentence containing such a pattern is the following:
%\begin{center}
\emph{``This paper deals with $\LogicHS$ \textbf{operators}
\myUnderline{meets}, \myUnderline{begins}, and \myUnderline{during} 
under homogeneity assumption.''}
%\end{center}

In such a toy example, a motivation for matching the word 
\textbf{operators} may be related to the fact that the noun preceding a natural language description of items may represent their type. In the above sentence, ``meets'', ``begins'', and ``during'' are indeed of type ``operators''. In such an interpretation, we are assuming that the  word denoting the type is put immediately before the list of words and thus conjunctions like, e.g., ``such as'' or ``like'' are not contemplated. However, they may be captured by regular expressions longer, but not much more complex, than the one we are going to 
show. For the sake of simplicity, we assume that the number of words in 
the list is greater than or equal to $3$ and each word is a single one.
As an example, the pattern \emph{``Concepts such \textbf{as} \myUnderline{atoms}, \myUnderline{compass structures}, and \myUnderline{requests} will be introduced in this section''} is not captured. A regular expression 
$\mathtt{re}$, which works in any modern programming language, 
that captures such a pattern is:
\[
   \mathtt{re} = \mathtt{(\escapebackslash w+)(?=\respace(?:\escapebackslash w+,\respace)\{2,\}}and\mathtt{\respace\escapebackslash w+)}
\]
\noindent where $\respace$ is used to highlight the single white space `` ''. Since it is outside the scope of this paper, we will not delve too much into the syntax of this kind of regular expressions. For that matter, wonderful websites such as \cite{Regexp101}, exist (they provide a quick reference for syntax and semantics together with examples and, more importantly, a full on-line environment for testing and debugging regular expressions). 

Let us briefly explain how  $\mathtt{re}$ captures the desired pattern.
First of all, we have that $\mathtt{(e)}$ is used to capture any pattern in $e$. The $\mathtt{(?= e )}$ operator checks whether the current position is followed by a pattern belonging to the language of $e$. The $\escapebackslash w$ variable represents any word-character, both lower and upper case. The operator $+$ is analogous to the operator $e^+ = ee^*$ in standard regular expressions. Thus, $\escapebackslash w+$ means any single word. The operator $(e)\{n,\}$,
with $n \geq 0$, captures a sequence of $n$ or more occurrences of pattern $e$. Finally, the operator $(?: e)$ represents just standard parentheses. 
A graphical account of the various parts of
regular expression $re$ is shown in Figure~\ref{fig:re}.

\begin{figure}
\begin{tikzpicture}[anchor=west]

\tikzset{explain/.style = {opacity=0.7} }
\tikzset{block/.style = {draw, rectangle} }


\node(RE0){$\mathtt{(\escapebackslash w+)}$};
\node(RE1) at (RE0.east) {$\mathtt{(?=}$};
\node(RE2) at (RE1.east) {$\mathtt{\respace}$};
\node(RE3) at (RE2.east) {$\mathtt{(?:\escapebackslash w+,\respace)\{2,\}}$};
\node(RE4) at (RE3.east) {$\mathtt{and\mathtt{\respace\escapebackslash w+}}$};
\node(RE5) at (RE4.east) {$\mathtt{)}$};

\draw [decorate,decoration={brace,amplitude=5pt,aspect=0.5}]
   ($(RE0.north west)$) -- node[above=4.5pt, inner sep=0](B1) {}
   ($(RE0.north east)$) ;

\draw [decorate,decoration={brace,amplitude=5pt,aspect=0.5}]
   ($(RE1.north west)$) -- node[above=4.5pt, inner sep=0](B2) {}
   ($(RE5.north east)$) ;

\draw [decorate,decoration={brace,amplitude=5pt,aspect=0.5, mirror, raise=0.1cm}]
   ($(RE2.south west)$) -- node[below=4.5pt, inner sep=0](B3) {}
   ($(RE2.south east)$) ;   

\draw [decorate,decoration={brace,amplitude=5pt,aspect=0.5, mirror}]
   ($(RE3.south west)$) -- node[below=4.5pt, inner sep=0](B4) {}
   ($(RE3.south east)$) ;

\draw [decorate,decoration={brace,amplitude=5pt,aspect=0.5, mirror}]
   ($(RE4.south west)$) -- node[below=4.5pt, inner sep=0](B5) {}
   ($(RE4.south east)$) ;   

\node[explain](EX0) at (8.25,2) {A };
\node[block](EX1) at (EX0.east){ single word is matched };
\node[explain, anchor=north west](EX2) at (EX0.south west) {if and only if it is};
\node[block, anchor=north west](EX3) at (EX2.south west) {immediately followed by};
\node[explain, anchor=north west](EX4) at (EX3.south west) {a concatenation of the following};
\node[explain, anchor=north west](EX5) at (EX4.south west) {three elements:};
\node[block, anchor=north west](EX6) at (EX5.south west) {
   (i) \begin{tabular}{l}a whitespace;\end{tabular}
};
\node[block, anchor=north west](EX7) at (EX6.south west) {
   (ii) \begin{tabular}{l}
   a sequence of two or more\\ concatenations of a single\\ word, a comma, and\\ a whitespace; 
   \end{tabular}
};
\node[block, anchor=north west](EX8) at (EX7.south west) {
   (iii) \begin{tabular}{l}the concatenation of  \\
    the word ``and'', a whitespace,\\ and a single word.\end{tabular}
};


\draw(B1) edge[looseness=0.6, out=90] (EX1.west);
\draw(B2) edge[looseness=0.7, out=90] (EX3.west);

\draw(B3) edge[looseness=0.7, out=-90] (EX6.west);
\draw(B4) edge[looseness=0.7, out=-90] (EX7.west);
\draw(B5) edge[looseness=0.7, out=-90] (EX8.west);


\end{tikzpicture}
\caption{\label{fig:re}
A graphical account of $re$ and its sub-expressions.
}
\end{figure}


Let $\Sigma = W \cup S$, where $W =\{a, \ldots, z, A, \ldots, Z \}$ (word symbols) and $S = \{\respace, \mathtt{.}, \mbox{`} \mathtt{,} \mbox{'} \}$ (separator symbols).
%
For the sake of brevity, we omit the intermediate phase of translating $re$ into our $*$-free restricted fragment and we jump directly to the translation into $\mathsf{BDA}_{hom}$. For the sake of simplicity, we do not apply the literal translation here; instead, we make use of a shorter, more understandable encoding which is tailored to the structure of the
specific regular expression $re$. As a preliminary step, we provide some shorthands and assumptions that make the encoding formulas more compact. First, we introduce a global modality $[G] \psi$, whose semantics is as follows: given a model $\bfM=(\bI_N, \cV)$, $\bfM, [0,y] \models [G] \psi$ if and only if $\psi \in \cV([x',y'])$ for every $0\leq x' \leq y' \leq N$, that is, if $[G] \psi$ holds on an initial interval of the model (an interval whose left endopoint is $0$), then $\psi$ holds on every interval of the model. In $\LogicABDhom$, we may capture the semantics of $[G]\psi$ by means of the formula $\psi \wedge \hsAA \psi \wedge \hsAA\hsAA \psi \wedge \hsAB \psi \wedge \hsAB\hsAA \psi$.
Moreover, in the encoding, we will make use of the 
shorthands $len_{\geq n}$ and $len_n$  for any $n \in \bN$, that constrain the length of the interval on which they hold to be greater than or equal to $n$ and exactly equal to $n$, respectively.
More precisely, given a model $\bfM=(\bI_N, \cV)$, we have that $[x,y] \models len_{\geq n}$ if and only if $y - x \geq n$,
and $\bfM, [x,y] \models len_n$ if and only if $y - x = n$.
In $\LogicABDhom$, we may capture the semantics of
$len_{\geq n}$ and $len_n$ by means of the formulas $\hsEB^n \pi$ and $len_{\geq n} \wedge \hsAB^{n + 1} \bot$, respectively.\footnote{Notice that we provide  a unary encoding of the length constraints. It is possible to make a binary encoding analogous to the one proposed in \cite {DBLP:journals/lmcs/BozzelliMMPS22}.}
Since in the proposed encoding we will make use of
proposition letters in $\Sigma$ to represent words as points of an interval model (Figure~\ref{fig:reinterval}), we need to force each point to hold \emph{exactly} one symbol
$\sigma \in \Sigma$. Such a constraint is imposed
by putting the formula $[G]( \pi \rightarrow 
\bigvee_{\sigma \in \Sigma}
(\sigma \wedge \bigwedge_{\sigma' \in \Sigma \setminus \{\sigma'\}  } \neg \sigma' ) )$ in conjunction with the encoding of $re$. For the sake of brevity, we will tacitly assume that this is the case. Finally, with a little abuse of notation, in the encoding of $re$ we will make use of $W$ as a shorthand for $\bigvee_{\sigma \in W} \sigma$, which basically allow us to state that a certain (point-)interval
holds a word symbol. 

Now, we are ready to encode $re$ by a formula $\psi_{re}$. More precisely, we will make
use of $\hsED\psi_{re}$ as the main formula, where $\psi_{re}$ just encodes the matching part. Thus, by 
``reading'' a model $\bfM=(\bI_N, \cV)$ for $\hsED\psi_{re},$ we can easily retrieve every
matching by taking all and only those intervals  $[x,y]$ such that $\bfM,[x,y]\models \psi_{re}$.
As an example, in Figure~\ref{fig:reinterval} we have that $\bfM, [0,90] \models \hsED \psi_{re}$, while $\
[24,34] \models \psi_{re}$. In fact, $[24,34]$ is the only interval that satisfies $\psi_{re}$ in the
model of Figure~\ref{fig:reinterval} and, as we will see when we will discuss $\psi_{re}$ in more detail, this is determined both by the points belonging to $[24,34]$ and by the formulas that hold in its ``right context'', that is, the intervals $[x,y]$, with $34\leq x \leq 90$. 

Let $\psi_{re} = \psi^{gm}_{w^+} \wedge
\hsEA(\psi_{\respace(w^,\respace)^{2+}} \wedge  \hsEA \psi^{gm}_{and\respace w^+} )$. Intuitively,
$\psi_{re}$ requires the presence of three adjacent intervals $[x,y], [y,z],$ and $[z, w]$ such that $\bfM,[x,y]\models \psi^{gm}_{w^+}$, $\bfM,[y,z]\models \psi_{\respace(w^,\respace)^{2+}}$, and $\bfM,[z,w]\models 
\psi^{gm}_{and\respace w^+}$. These sub-formulas constrain the three regular expressions whose concatenation forms $re$ as follows: 

\smallskip

\begin{compactitem}

\item $\psi^{gm}_{w^+}=\hsEB\neg W \wedge \hsAB(len_{\geq 1} \rightarrow \hsEA W)
\wedge \hsEB\hsEA W \wedge \hsEA \neg W$. This formula holds over an interval $[x,y]$ if and only if point-intervals $[x,x]$ and $[y,y]$ do not hold a word symbol (conjuncts $\hsEB\neg W$ and $\hsEA \neg
W$, respectively), but a word symbol holds at all the internal point-intervals $[x',x']$, with $x<x'<y$  (conjunct $\hsAB(len_{\geq 1} \rightarrow \hsEA W)$). Finally, it constrains the interval $[x,y]$ to contain at least one word symbol (conjunct $\hsEB\hsEA W$). Intuitively,  $\psi^{gm}_{w^+}$ encodes the greedy match (gm) of a single non-empty word preceeded and followed by two singleton separator symbols. as an example, in Figure \ref{fig:reinterval}, we have that $\psi^{gm}_{w^+}$ holds over the interval $[24,34]$.

\item 
$\psi_{\respace(w^+,\respace)^{2+}} = \hsEA \respace \wedge \hsEB (len_1 \wedge \hsEB \respace \wedge \hsEA W)
\wedge \hsAD(len_1 \rightarrow (\hsEB \respace \wedge \hsEA W) \vee (\hsEB , \wedge \hsEA \respace) \vee (\hsEB
W \wedge \hsEA W) \vee (\hsEB W \wedge \hsEA ,)) \wedge \hsEB(\hsEA ,\wedge  \hsEB\hsEA ,)$. This formula holds over an interval $[x,y]$ if and only if
all the following conditions hold:

\smallskip

\begin{compactenum}

\item the symbol $\respace$ holds on point-interval $[x,x]$ and a word symbol holds on point-interval $[x+1,x+1]$ (conjunct $\hsEB (len_1 \wedge \hsEB \respace \wedge \hsEA W)$); 

\item the symbol $\respace$ holds on point-interval $[y,y]$  (conjunct $\hsEA \respace$);
%
\item for every strict sub-interval of $[x,y]$ of the form $[x', x'+1]$, we have that either $[x',x']$ is labelled with $\respace$ and $[x'+1, x'+1]$ 
by a word symbol (disjunct $\hsEB \respace \wedge \hsEA W$), or
$[x',x']$ is labelled with ``$,$'' and $[x'+1, x'+1]$ 
with $\respace$  (disjunct $\hsEB , \wedge \hsEA \respace$), or
both $[x',x']$ and $[x'+1, x'+1]$ 
are labelled with a word symbol (disjunct $\hsEB W \wedge \hsEA W$),  or
$[x',x']$ is labelled with a word symbol  and $[x'+1, x'+1]$ 
with ``$,$'' (disjunct $\hsEB W \wedge \hsEA ,$); 

\item the symbol ``$,$'' appears as a label of  \emph{at least} two distinct point-intervals 
$[x',x']$ and $[x'', x'']$ in $[x,y]$, i.e., with
 $x< x'< x''<y$  (conjunct $\hsEB(\hsEA ,\wedge \hsEB\hsEA ,)$).
 In Figure~\ref{fig:reinterval}, such a condition is satisfied by point-intervals $[40,40]$ and $[48,48]$, which are included in the interval $[34,49]$.

\end{compactenum}

\smallskip

Intuitively, the conjunct $\hsAD(len_1 \rightarrow (\hsEB \respace \wedge \hsEA W) \vee (\hsEB , \wedge \hsEA \respace) \vee (\hsEB W \wedge \hsEA W) \vee (\hsEB W \wedge \hsEA ,))$ constrains the word underlying $[x+1, y+1]$ to belong to the language of $((w)^+, \respace)^*$, while the conjunct $\hsEB(\hsEA , \hsEB\hsEA ,)$ forces at least two iterations of the $*$ operation in such a language. Thus, together they force  such a word to belong to $((w)^+, \respace)^{2+}$;

\item $\psi^{gm}_{and\respace w^+} =  \hsEB a
\wedge \hsEB(len_1 \wedge \hsEA n)
\wedge \hsEB(len_2 \wedge \hsEA d)
\wedge \hsEB(len_3 \wedge \hsEA \respace)
 \wedge \hsEB(len_{\geq 4} \rightarrow \hsEA W) \wedge \hsEA \neg W$. This formula holds over an interval $[x,y]$ if and only if the word underlying the interval $[x, x + 3]$ is exactly ``$and\respace$'' (conjuncts $\hsEB a$,
$\hsEB(len_1 \wedge \hsEA n)$,
$\wedge \hsEB(len_2 \wedge \hsEA d)$, and 
$\wedge \hsEB(len_3 \wedge \hsEA \respace)$) followed by an uninterrupted sequence of word symbols 
underlying the interval $[x+4, y-1]$ (conjunct $\hsEB(len_{\geq 4} \rightarrow \hsEA W)$).
In addition, it imposes the word underlying the interval $[x+4, y-1]$ to be a greedy match, that is, 
an entire word is captured,  since we force a separator symbol on $[y+1, y+1]$ by means of the conjunct $\hsEA \neg W$.

\end{compactitem}

\begin{figure}
\begin{tikzpicture}
   \begin{scope}[node distance=0.3cm]


\node[opacity=0.5,draw, circle, inner sep=1, 
label={[scale=1, opacity=0.5,]180:$\scalebox{0.525}{$\ldots$}$},
label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 22 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ H $}$}](22-22) [] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 23 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ S $}$}
      ](23-23) [right of=22-22] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 24 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ \respace $}$}](24-24) [right of=23-23] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 25 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ o $}$}](25-25) [right of=24-24] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 26 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ p $}$}](26-26) [right of=25-25] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 27 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ e $}$}](27-27) [right of=26-26] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 28 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ r $}$}](28-28) [right of=27-27] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 29 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ a $}$}](29-29) [right of=28-28] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 30 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ t $}$}](30-30) [right of=29-29] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 31 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ o $}$}](31-31) [right of=30-30] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 32 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ r $}$}](32-32) [right of=31-31] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 33 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ s $}$}](33-33) [right of=32-32] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 34 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ \respace $}$}](34-34) [right of=33-33] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 35 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ m $}$}](35-35) [right of=34-34] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 36 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ e $}$}](36-36) [right of=35-35] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 37 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ e $}$}](37-37) [right of=36-36] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 38 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ t $}$}](38-38) [right of=37-37] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 39 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ s $}$}](39-39) [right of=38-38] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 40 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ , $}$}](40-40) [right of=39-39] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 41 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ \respace $}$}](41-41) [right of=40-40] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 42 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ b $}$}](42-42) [right of=41-41] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 43 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ e $}$}](43-43) [right of=42-42] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 44 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ g $}$}](44-44) [right of=43-43] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 45 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ i $}$}](45-45) [right of=44-44] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 46 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ n $}$}](46-46) [right of=45-45] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 47 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ s $}$}](47-47) [right of=46-46] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 48 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ , $}$}](48-48) [right of=47-47] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 49 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ \respace $}$}](49-49) [right of=48-48] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 50 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ a $}$}](50-50) [right of=49-49] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 51 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ n $}$}](51-51) [right of=50-50] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 52 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ d $}$}](52-52) [right of=51-51] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 53 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ \respace $}$}](53-53) [right of=52-52] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 54 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ d $}$}](54-54) [right of=53-53] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 55 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ u $}$}](55-55) [right of=54-54] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 56 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ r $}$}](56-56) [right of=55-55] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 57 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ i $}$}](57-57) [right of=56-56] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 58 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ n $}$}](58-58) [right of=57-57] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 59 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ g $}$}](59-59) [right of=58-58] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 60 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ \respace $}$}](60-60) [right of=59-59] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 61 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ u $}$}](61-61) [right of=60-60] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 62 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ n $}$}](62-62) [right of=61-61] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 63 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ d $}$}](63-63) [right of=62-62] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 64 $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ e $}$}](64-64) [right of=63-63] {};
      

\node[opacity=0.5,draw, circle, inner sep=1, label={[scale=1, opacity=0.5,]270:$\scalebox{0.525}{$ 65 $}$},
label={[scale=1, opacity=0.5,]0:$\scalebox{0.525}{$ \ldots $}$},
      label={[scale=1, opacity=0.5,]90:$\scalebox{0.525}{$ r $}$}](65-65) [right of=64-64] {};
      
\def\y{2cm}
\draw[-] ($(25-25)+(0, \y)$) -- ($(63-63)+ (0, \y)$)
node[fill=white, pos=0.5] {\scalebox{0.75}{$\hsED \psi_{re}$}}; 
\draw[dashed] ($(25-25)+(0, \y)$) -- ($(25-25)+(-1, \y)$);    
\draw[dashed] ($(63-63)+(0, \y)$) -- ($(63-63)+(1, \y)$);    


\def\y{1cm}
\def\b{24}
\def\e{34}
\draw[|-|] ($(\b-\b)+(0, \y)$) -- ($(\e-\e)+ (0, \y)$)
node[fill=white, pos=0.5] {\scalebox{0.75}{$\psi_{re}, \psi^{gm}_{w^+}$}};

\def\y{1cm}
\def\b{34}
\def\e{49}
\draw[|-|] ($(\b-\b)+(0, \y)$) -- ($(\e-\e)+ (0, \y)$)
node[fill=white, pos=0.5] {\scalebox{0.75}{$\psi_{\respace(w^+,\respace)^{2+}}$}};

\def\y{1cm}
\def\b{49}
\def\e{60}
\draw[|-|] ($(\b-\b)+(0, \y)$) -- ($(\e-\e)+ (0, \y)$)
node[fill=white, pos=0.5] {\scalebox{0.75}{$\psi_{and\respace w^+}$}};

  \end{scope}

\end{tikzpicture}
\caption{\label{fig:reinterval} a graphical account of how a $\hsED \psi_{re}$
 holds over an interval model representing a text.}
\end{figure}

\smallskip

We conclude the section with some remarks about the practical use of regular expressions. To the best of our knowledge, in their implementation the majority of existing programming languages do not support the free use of negation in regular expressions, but they allow for positive/negative lookahead/lookbehind. In this section, we showed how to deal with positive/negative lookahead by means of modality $\hsEA$. Moreover, we argued that positive/negative lookbehind may be captured by adding  modality $\hsEAbar$, which is the converse of modality $\hsEA$, to $\mathsf{BDA}_{hom}$, thus obtaining the logic $\mathsf{BDA\overline{A}}_{hom}$. 
%
For the sake of simplicity, we did not take modality $\hsEAbar$ into consideration
in this work, as its introduction involves a number of  technicalities. However, in view of the results 
established in the next section, we may conjecture with a certain confidence that, under the homogeneity assumption, the satisfiability problem for $\mathsf{BDA\overline{A}}_{hom}$ belongs to the same complexity class as its proper fragment $\mathsf{BDA}_{hom}$.


==> conclusion.tex <==
%!TEX root = ./main.tex


\section{Conclusions}\label{sec:conclusions}

In this paper, we proved that, under the homogeneity assumption, the satisfiability checking problem for $\mathsf{BDA}_{hom}$, over finite  linear orders,
is EXPSPACE-complete. This result stems a number of observations
about the complexity landscape of the satisfiability and 
model checking problems for $\mathsf{HS}$ fragments under homogeneity ($\mathsf{HS}_{hom}$):
\begin{inparaenum}
\item it improves the previously-known non-elementary upper bound 
\cite{DBLP:journals/acta/MolinariMMPP16};
\item it identifies the first EXPSPACE-complete fragment of 
$\mathsf{HS}_{hom}$ with respect to the satisfiability problem
\cite{DBLP:journals/tcs/BozzelliMMPS19}.
\end{inparaenum}

For what concerns the satisfiability problem for $\textsf{BDA}_{hom}$, we already observed that
the homogeneity assumption plays a crucial role only in the proof of the EXPSPACE membership of the problem (upper bound), while it does not play any role in the proof of the EXPSACE-hardness of the problem (lower bound).

The results for $\mathsf{BDA}_{hom}$ also shed some light on the problem of determining the exact complexity of the satisfiability checking problem for 
 $\mathsf{BE}_{hom}$, which is still open. As a matter of fact, $\mathsf{BDA}_{hom}$
and  $\mathsf{BE}_{hom}$ are not comparable from the point of view of their expressiveness \cite{DBLP:journals/tcs/BresolinMMSS14}.
However, $\mathsf{BDA}_{hom}$ captures
a fragment of $\mathsf{BE}_{hom}$, that is, $\mathsf{BD}_{hom}$ extended with a restricted version of modality $\hsEE$, namely, $\hsEE_{\pi} \psi = \hsEA(\pi \wedge \psi)$, that allows one to predicate on the right endpoint of an interval. As shown in Section~\ref{sec:hardness}, this is the key property 
that causes the increase in complexity of the satisfiability checking problem from $\mathsf{BD}_{hom}$ (PSPACE-complete)
to $\mathsf{BDA}_{hom}$ (EXPSPACE-complete). 
It is easy to see that the result given here 
can be easily extended to the case of homogeneous 
structures isomorphic to $\bbN$.

From a more practical standpoint, we showed how $\textsf{BDA}_{hom}$ may encode a very expressive fragment of generalized $*$-free regular expression, namely, the fragment that features prefix, infix, and lookahead. Thanks to the result obtained
in this work, we have that the emptiness problem for the languages expressed by means of 
such a fragment is elementary (EXPSPACE-complete)
in constrast to the non-elementary-hard result which was  known for the the emptiness problem for full generalized $*$-free regular expression
\cite{stockmeyer1974complexity}.

As for future work, we plan to investigate the satisfiability/model checking problems for (fragments of) $\mathsf{HS}_{hom}$, interpreted over the linear orders $\bbQ$
and $\bbR$. However, the precise characterization of the complexity of the satisfiability problem for $\mathsf{BE}_{hom}$ remains the main open problem on the path to determining the exact complexity of the satisfiability problem for full $\mathsf{HS}_{hom}$ over finite linear orders.



==> expspace.tex <==
%!Tex root = ./main.tex

\section{The satisfiability problem for
\texorpdfstring{$\mathsf{BD}_{hom}$}{} is decidable in EXPSPACE}
\label{sec:expspace}

In this section, by exploiting the properties proved in Section~\ref{sec:properties}, we show that the problem of checking whether a $\mathsf{BD}_{hom}$ formula $\varphi$ is satisfied by some homogeneous model can be decided in exponential space. 
%
First, by means of a suitable small model theorem, we prove
that either $\varphi$ is unsatisfiable or it is satisfied 
by a model (a compass structure) of at most doubly-exponential  size in $|\varphi|$; then, we show that this model of doubly-exponential size can be guessed in single exponential space.

\begin{theorem}\label{thm:bound2}
Let $\varphi$ be a $\mathsf{BD}_{hom}$ formula. 
The problem of deciding whether or not it is 
satisfiable belongs to EXPSPACE.
\end{theorem}
The proof of Theorem \ref{thm:bound2} follows from
Corollary \ref{cor:coveredismonotone}, Lemma \ref{thm:smallcompass}, and Lemma \ref{thm:bound1} below.

First of all, thanks to the property proved in Section \ref{subsec:covered}, we know that, for every row $y$, there is a finite set of columns $C_y = \{x_1, \ldots, x_n\}$ that behave pairwise differently for the portion of the compass structure above $y$. This means that each column $0\leq x\leq y$, with $x \notin C_y$, behaves exactly as some $x_i \in C_y$ 
    above $y$, that is, for all $y'> y$, $\cL(x,y')=\cL(x_i,y')$. We prove that $n$ is bounded by $|\varphi|$, from which it immediately follows that, in any large enough model,
    there are two rows $y$ and $y'$, with 
    $\shadingG(x)[y'] = 
  \shadingG(x_0)[y']$. Then, we can suitably contract the model into one whose $Y$-size is $y'-y$ shorter. By (possibly) repeatedly applying such a contraction, we  obtain a model whose $Y$-size satisfies a doubly exponential bound. To complete the proof, it suffices to show that there exists a procedure that checks whether or not such a model exists in exponential space.

\input{\detokenize{properties_contraction}}











==> properties.tex <==
%!Tex root = ./main.tex

\section{Spatial properties of compass structures for 
\texorpdfstring{$\mathsf{BD}_{hom}$} \ \ formulas}
\label{sec:properties}

In this section, we prove a series of spatial properties of compass structures that turn out to be very useful in the proofs of 
the results of Sections \ref{sec:expspace} and \ref{sec:abdexpspace}.  
%
Each property is proved by making use of the 
previous one as follows:

\begin{compactitem}

    \item[Section \ref{subsec:columns} - ] We  first show that for any compass structure and any of its $X$-axis coordinate $x$, the sequence $\cL(x,0)\ldots\cL(x,N)$ is monotonic, that is, for any triplet $0\leq y_1 < y_2 < y_3 \leq N$, it cannot be the case that $\cL(x,y_1)= \cL(x,y_3)$ and $\cL(x, y_1) \neq \cL(x, y_2)$. Such a property allows us to represent relevant information associated with any column $x$ in space (polynomially) bounded in $|\varphi|$.
    
    \item[Section \ref{subsec:equivcolumns} - ]  Next, we define an equivalence relation over columns 
    such that two columns are equivalent if they feature the same set of atoms. It is easy to verify that such an equivalence relation is of finite index and its index is  exponentially  bounded in $|\varphi|$. By exploiting the representation of Section \ref{subsec:columns}, we first define a partial order  
    over equivalent columns, and then we prove that, in a compass structure,  such  a relation totally orders equivalent columns.
    
    \item[Section \ref{subsec:covered} - ]  By exploiting the total order of the elements of each equivalence class, we show a crucial property of the rows of a compass structure, which is the cornerstone of the proof. First, we associate with each point $(x,y)$ on row $y$, with $0\leq x \leq y$, a tuple consisting of: (i) $\cL(x,y)$, (ii) the equivalence class $\sim_x$ of column $x$, and (iii) the set of pairs $(\cL(x',y), \sim_{x'})$, for all %$x'$ with 
    $x < x' \leq y$, and then we prove that, for every pair of points $(x,y), (x',y)$ that feature the same tuple, $\cL(x,y') = \cL(x', y')$ for all $y'>y$, that is, columns $x$ and $x'$ behave the same way (i.e., exhibit the same labelling) from $y$ to the upper end.

\end{compactitem}

\input{propertiesStep1}
\input{propertiesStep2}
\input{propertiesStep3}










